The Baum-Connes conjecture, Swan group actions and controlled topology

We give a new proof of some cases of the Baum-Connes conjecture along the lines of a proof of the Farrell-Jones conjecture.

==> chapters/SwanNil.tex <==
\section{The Swan group of the integers and Nil terms}

\subsection{Endomorphism and Nil categories}

\fxnote{Do it}

\subsection{The Swan group action and Nil terms}

Let $R$ be a ring. The (integral) Swan group $\Sw(\IZ)$ of $\IZ$ acts on the $K$-theory of $R\IZ  = R[t,t^{-1}]$. On the other hand, the Bass-Heller-Swan formula says that
\[
K_{*} R[t,t^{-1}]  \cong K_{*-1}(R) \oplus K_{*}(R) \oplus \Nil_{*-1}(R) \oplus \Nil_{*-1}(R)
\] 

We will show how the action of $\Sw(\IZ)$ on $K_{*} R[t,t^{-1}]$ decomposes into the direct summands on the right-hand side. \\
\fxnote{Swan(Z) = automorphism category}
Consider the category $P(R[t])$ of projective modules over $R[t]$. Given an element $M = (\IZ^{n}, f)$ of $\mod_{\IZ}(\IZ)$ and $P \in P(R[t])$, we obtain a new $R[t]$-module $M \otimes_{\Delta} P$, with $t$ acting diagonally as $t$ on $P$ and as $f$ on $M$. 

\begin{prop}
The module $M \otimes_{\Delta} P$ is again a projective $R[t]$-module.
\end{prop}

\begin{proof}
Since tensoring with $M$ preserves direct sums, it is enough to see that $M \otimes_{\Delta} R[t]$ is a free $R[t]$-module. Then the map
\begin{align*}
M \otimes_{r} R[t] &\rightarrow M \otimes_{\Delta} R[t] \\
m \otimes t^{k} &\mapsto f^{k}(m) \otimes t^{k}
\end{align*}
is an isomorphism of $R[t]$-modules, with inverse
\begin{align*}
M \otimes_{\Delta} R[t] &\rightarrow M \otimes_{r} R[t] \\
m \otimes t^{k} &\mapsto f^{-k}(m) \otimes t^{k}
\end{align*}
\end{proof}

Hence we obtain a biexact functor
\begin{align*}
\mod_{\IZ}(\IZ) \times P(R[t]) &\rightarrow P(R[t]) \\
(M,P) &\mapsto M \otimes_{\Delta} P
\end{align*}
and an induced action of $\Sw(\IZ)$ on $K_{*}(R[t])$. This is checked as in the proof of \ref{action}. 

\begin{prop}
The inclusion $R[t] \rightarrow R[t,t^{-1}]$ induces a $\Sw(\IZ)$-module map $K_{*}(R[t]) \rightarrow K_{*}(R[t,t^{-1}])$. 
\end{prop}

\begin{proof}
This is more or less clear from the definitions, since $(M \otimes_{\Delta} P) \otimes_{R[t]} R[t,t^{-1}] \cong M \otimes_{\Delta} (P \otimes_{R[t]} R[t,t^{-1}])$ as $R[t,t^{-1}]$-modules for any projective $R[t]$-module $P$.
\end{proof}

The Bass-Heller-Swan formula is an extension of an isomorphism
\[
K_{*}(R[t]) \cong K_{*}(R) \oplus \Nil_{*-1}(R)
\]
Once we understand how the $\Sw(\IZ)$-action on $K_{*}(R[t])$ decomposes with respect to this decomposition, it is not hard to derive the desired decomposition on $K_{*}(R[t,t^{-1}])$, so let us set out to do this. For this, we need to understand how the isomorphism $K_{*}(R[t]) \cong K_{*}(R) \oplus \Nil_{*-1}(R)$ comes about. 

\begin{definition}
Let $\Mod(\IP_{R}^{1})$ be the following category: Objects are triples $(M^{+}, M^{-}, \theta)$ with $M^{+}$ a finitely generated $R[t]$-module, $M^{-}$ a finitely generated $R[t^{-1}]$-module and $\theta: M^{+} \otimes_{R[t]} R[t,t^{-1}] \rightarrow M^{-} \otimes_{R[t^{-1}]} R[t,t^{-1}]$ an isomorphism. A morphism $f: (M^{+}, M^{-}, \theta) \rightarrow (N^{+}, N^{-}, \phi)$ consists of two morphisms $f^{\pm}: M^{\pm} \rightarrow N^{\pm}$ such that the diagram
\[
\xymatrix{
M^{+} \otimes_{R[t]} R[t,t^{-1}] \ar[dd]^{f^{+} \otimes 1} \ar[rr]^{\theta} & & M^{-} \otimes_{R[t^{-1}]} R[t,t^{-1}] \ar[dd]^{f^{-1} \otimes 1} \\
\\
 N^{+} \otimes_{R[t]} R[t,t^{-1}] \ar[rr]^{\phi} & & N^{-} \otimes_{R[t]} R[t,t^{-1}] \\
 }
\]
This is an abelian category, with direct sums, kernels and cokernels formed pointwise. Let $P(\IP_{R}^{1})$ be the full subcategory on those objects $(M^{+}, M^{-}, \theta)$ with $M^{+}$ and $M^{-}$ projective. \fxnote{Is this the same as projective in the abelian category?}
 \end{definition}
 
Let $u_{0}: P(R) \rightarrow P(\IP_{R}^{1})$ be the functor sending an $R$-module $P$ to $(P \otimes_{R} R[t], P \otimes_{R} R[t^{-1}], \id)$ and 
$u_{1}:  P(R) \rightarrow P(\IP_{R}^{1})$ be the functor sending $P$ to  $(P \otimes_{R} R[t], P \otimes_{R} R[t^{-1}], t \cdot -)$. The following is proven in \cite[9.11]{Swan}:

\begin{thm}
The functors $u_{0}, u_{1}$ induce an isomorphism
\[
(u_{0}, u_{1}): K_{*}(P(R)) \oplus K_{*}(P(R)) \rightarrow K_{*}(P(\IP_{R}^{1}))
\]
\end{thm}
 
\begin{definition}
Let $P^{-} = P^{-1}(\IP_{R}^{1})$ be the full subcategory of $\mod(\IP_{R}^{1})$ spanned by the objects $(M^{+}, M^{-}, \alpha)$ such that $M^{-}$ is a projective $R[t^{-1}]$-module and $M^{+}$ has a resolution of length one by projective $R[t]$-modules and let $\calh$ be the full subcategory of $P^{-}$ spanned by the objects $(M^{+}, M^{-}, \theta)$ with $M^{-} =  0$. Let $F: P^{-} \rightarrow P(R[t^{-1}])$ be the functor sending $(M^{+}, M^{-}, \theta)$ to $M^{-}$.
\end{definition}

The following is \cite[9.14]{Swan} and an application of the resolution theorem \cite[5.3.25]{Ros}.

\begin{thm}
The sequence of categories
\[
\calh \rightarrow P^{-} \rightarrow P(R[t^{-1}])
\]
induces a homotopy fibration in $K$-theory, and the inclusion $P(\IP_{R}^{1}) \rightarrow P^{-}$ is a $K$-equivalence.
\end{thm}

The link to the Nil groups is given by the following proposition; compare \cite[10.7]{Swan}.

\begin{prop}
The category $H^{-}$ is equivalent to $\Nil(R)$.
\end{prop}

\begin{proof}
Let $(M^{+}, 0, \theta)$ be an object of $H^{-}$. We first argue that $M^{+}$ is a finitely generated projective $R$-module. Since $M$ is finitely generated as $R[t]$-module and vanishes after inverting $t$, there must be an $n > 0$ with $t^{n}M = 0$.  Hence $M$ is a finitely generated $R[t]/t^{n}$-module and then also a finitely generated $R$-module. \\
Now we turn to projectivity. By definition, there are projective $R[t]$-modules $P$ and $Q$ and a short exact sequence $0 \rightarrow Q \rightarrow P \rightarrow M \rightarrow 0$. 
Now also $M \cong t^{n}P/t^{n}Q$. Set $A = t^{n}Q$, $B = t^{n}P$ and $C = Q$. We have $A \subset B \subset C$ and a short exact sequence
\[
0 \rightarrow B/A \rightarrow C/A \rightarrow C/B \rightarrow 0
\]
The middle modul $Q/t^{n}Q$ is projective over $R[t]/t^{n}$ since $Q$ is projective over $R[t]$; it then easily follows that $Q/t^{n}Q$ is projective over $R$ since any epimorphism of $R$-modules $X \rightarrow Y$ is also an epimorphism of $R[t]/t^{n}$-modules by letting $t$ act as $0$.The right-hand module is of projective dimension at most $1$ over $R[t]$ and hence over $R$. To prove that $B/A$ is projective, we can now compute $\Ext_{i}(B/A,-)$. Since $\Ext_{i}(C/B,-) = 0$ for $i > 1$, this is a direct consequence of the long exact sequence of $\Ext$-groups associated to the short exact sequence $0 \rightarrow B/A \rightarrow C/A \rightarrow C/B \rightarrow 0$. \\
Now define a functor $F: \calh \rightarrow \Nil(R)$ by sending $(M^{+}, 0, 0)$ to $(M^{+}, t)$. This is well-defined since $M^{+}$ is finitely generated projective as an $R$-module. Its inverse is given by sending $(P,f) \in \Nil(R)$ to $(P,0,0)$ where we view $P$ as an $R[t]$-module via $f$. To see that $(P,0,0) \in \calh$, note that we have the characteristic sequence
\[
0 \rightarrow P[t] \stackrel{t-f}{\rightarrow} P[t] \rightarrow P \rightarrow 0
\]
Set $X = (P[t], P[t^{-1}], t)$ and $Y = (P[t], P[t^{-1}], \id)$. The map $(t-f, 1-t^{-1}f): X \rightarrow Y$ gives the desired resolution $0 \rightarrow X \rightarrow Y \rightarrow (P,0,0) \rightarrow 0$ with $X,Y \in P(\IP_{R}^{1})$. 
\end{proof}

We hence get a long exact sequence
\[
\cdots K_{n}(\Nil(R)) \rightarrow K_{n}(R) \oplus K_{n}(R) \rightarrow K_{n}(R[t^{-1}]) \rightarrow K_{n-1}(\Nil R) \rightarrow \cdots
\]
where we identify $K_{n}(R) \oplus K_{n}(R)$ with $K_{n}(P^{-1})$ via $u_{0}$ and $u_{1}$. We can now decompose this sequence further. On the first $K_{n}(R)$-summand in $K_{n}(R) \oplus K_{n}(R)$, the map to $K_{n}(R[t^{-1}])$ is the map induced by the inclusion $R \rightarrow R[t^{-1}]$, and on the anti-diagonal summand $\{(v,-v) \mid v \in K_{n}(R)\}$, the map is zero. Hence we can split the sequence to get
\[
0 \rightarrow K_{n}(R) \rightarrow K_{n}(R[t^{-1}] \rightarrow K_{n-1}(\Nil(R)) \rightarrow K_{n-1}(R) \rightarrow 0
\]
where the first $K_{n}(R)$ is the first summand of $K_{n}(R) \oplus K_{n}(R)$ and the last is the anti-diagonal one. It remains to identify the map $K_{n-1}(\Nil(R)) \rightarrow K_{n-1}(R)$. We have three functors from $\Nil(R)$ to $P(\IP_{R}^{1})$: The functor $F$ sending $(M,f)$ to $(M,0,0)$ which we are interested in, the functor $F_{1}$ sending $(M,f)$ to
\[
u_{1}(M) = (M[t], M[t^{-1}], t)
\]
which ignores the $f$, and the corresping functor $F_{0}$ sending $M$ to
\[
u_{0}(M) = (M[t], M[t^{-1}], \id)
\]
For $(M,f) \in \Nil(R)$, the map $(t-f,1-t^{-1}f): u_{1}(M) \rightarrow u_{0}(M)$ gives rise to a short exact sequence of functors
\[
0 \rightarrow F_{1} \rightarrow F_{0} \rightarrow F \rightarrow 0
\]
By the additivity theorem, this implies that $K_{*}(F) = K_{*}(F_{0})-K_{*}(F_{1})$. Since $u_{0}$ and $u_{1}$ also give the identification $K_{*}(\IP_{R}^{1}) \cong K_{*}(R) \oplus K_{*}(R)$, we find that $K_{*}(F)$ identifies with the $K$-theory of the evaluation functor $\Nil(R) \rightarrow P(R)$ composed with $u_{0}-u_{1}$. Altogether, we find that the map $K_{n-1}(\Nil(R)) \rightarrow K_{n-1}(R)$ is induced by the evaluation functor. Hence we get short exact sequences
\[
0 \rightarrow K_{n}(R) \rightarrow K_{n}(R[t^{-1}] \rightarrow \Nil_{n-1}(R) \rightarrow 0
\]
as desired.

\begin{definition}
Let $S = (\IZ^{n}, f) \in \mod_{\IZ}(\IZ)$. We define a functor $S \otimes -: P^{-} \rightarrow P^{-}$ as follows: Given an object $(M^{+}, M^{-}, \theta)$, we form the $R[t]$-module $S \otimes_{\Delta} M^{+}$, with $t$ acting diagonally and as $f$ on $S$. By the usual trick, if $M^{+}$ was projective, this yields a projective $R[t]$-module. Since tensoring with $S$ is exact, a resolution by projective modules is turned into a resolution by projective modules and hence we indeed land in $P^{-}$. In the same manner, let $S \otimes_{\Delta} M^{-}$ be the $R[t^{-1}]$-module obtained by letting $t^{-1}$ acting diagonally and as $f^{-1}$ on $S$. Then $\id \otimes \theta$ is an isomorphism from $(S \otimes_{\Delta} M^{+}) \otimes_{R[t]} R[t,t^{-1}]$ to  $(S \otimes_{\Delta} M^{-}) \otimes_{R[t^{-1}]} R[t,t^{-1}]$ since $(S \otimes_{\Delta} M^{+}) \otimes_{R[t]} R[t,t^{-1}]$ and $S \otimes_{\Delta} (M^{+} \otimes_{R[t]} R[t,t^{-1}])$ are canonically isomorphic, and similarly for $M^{-}$. This gives rise to a biexact functor
\begin{align*}
\mod_{\IZ} \times P^{-} &\rightarrow P^{-} \\
(S,(M^{+}, M^{-},\theta)) &\mapsto  (S \otimes_{\Delta} M^{+}, S \otimes_{\Delta} M^{-}, \id \otimes \theta)
\end{align*}
which restricts to $\calh \cong \Nil(R)$. The evaluation functor $P^{-} \rightarrow \IP(R[t^{-1}])$ is equivariant with respect to the biexact pairings of $\mod_{(\IZ, \IZ)}$ with the two categories.
\end{definition}

Altogether, we get the following result:

\begin{prop}
Equip $K_{n}(R)$ with the $\mod_{\IZ}$-action where a Swan module $S$ acts by multiplication with its dimension. Then the short exact sequence
\[
0 \rightarrow K_{n}(R) \rightarrow K_{n}(R[t^{-1}]) \rightarrow \Nil_{n-1}(R) \rightarrow 0
\]
is a short exact sequence of $\Sw(\IZ)$-modules. 
\end{prop}

\begin{proof}
That the right-hand map is equivariant is a formal consequence of the fact that we have actions of $\Sw(\IZ)$ on all three terms of the fiber sequence of which $K_{n}(R[t^{-1}] \rightarrow \Nil_{n-1}(R)$ is the boundary map. For the left-hand map, note that for a Swan module $S = (\IZ^{n}, \rho)$, the two functors $P(R) \rightarrow P(R[t^{-1}])$ obtained by first tensoring with $\IZ^{n}$ and then inducing up to $R[t^{-1}]$ or first inducing up and then tensoring diagonally with $S$ are isomorphic: For $R[t^{-1}]$ module homomorphisms which are induced up from $R$-modules, the isomorphism $S \otimes_{\Delta} P \cong S \otimes_{r} P$ is natural. This proves the claim for the first map.
\end{proof}

\fxnote{Bass-Heller-Swan decomposition?}

\subsection{The Witt Ring action on the Nil groups}

\begin{definition}
Let $B$ be an $R$-algebra. For $n \in \IN$, let $\Fil_{n} \Nil(B)$ be the full exact subcategory of $\Nil(R)$ spanned by the nilpotent endomorphisms $(P, f)$ such that $f^{n} = 0$. Let $\Fil_{n} \tilde{K_{*}} \Nil(B)$  be the image of $K_{*} \Fil_{n} \Nil(B)$ in $\tilde{K_{*}} \Nil(B)$.
\end{definition}



\begin{prop}
Let $B$  be an $R$-algebra. Let $(R^k, f)$ and $(R^{p}, g)$ be objects of $\End(R)$ such that $\chi(f) = \chi(g) \mod t^{n}$. Then the formal difference $(R^k, f)-(R^{p}, g)$ in $\bend_{0} (R)$ acts as $0$ on  $\Fil_{n} \tilde{K_{*}} \Nil(B)$.
\end{prop}

\begin{proof}
By adding appropriate zeros, we may assume $k = p$. It is enough to see that tensor product with $f-g$ induces the zero map on $ \tilde{K_{*}} \Fil_{n} \Nil(B)$. Let $k = n+m$. We may assume that $f$ has the form
\[
\begin{pmatrix}
0 & 0 & 0 & ... & -a_{n+m} \\
1& 0& 0&... & -a_{n+m-1} \\
0 & 1& 0 & ...& ... \\
... & ... &... & ... & ... \\
0 & 0 & 0 &...&-a_{1}
\end{pmatrix} 
\]
and similarly for $g$ with $a_{i}$ replaced by $b_{i}$. The assumption on $f$ and $g$ says that $a_{i} = b_{i}$ for $i < n$. \\
Now $R$ and also $B$ is a $C = \IZ [x_{1}, x_{2}, ... x_{n+m}]$-algebra with $x_{i}$ acting as multiplication with $a_{i}$. The objects of $\Fil_{n} \Nil(B)$ are then modules over the ring $C[y]/(y^{n})$, where $y$ acts on $(B,\nu)$ as $\nu$. We hence get a biexact pairing
\[
\Nil C[y]/(y^{n}) \times \Fil_{n} \Nil(B) \rightarrow \Fil_{n} \Nil(B)
\] 
by tensoring over $C[y]/(y^{n})$. Now consider the nilpotent matrix
\[
A = y\begin{pmatrix}
0 & 0 & 0 & ... & -x_{n+m} \\
1& 0& 0&... & -x_{n+m-1} \\
0 & 1& 0 & ...& ... \\
... & ... &... & ... & ... \\
0 & 0 & 0 &...&-x_{1}
\end{pmatrix} 
\]
as an endomorphism of $(C[y]/(y^{n}))^{n+m}$. The functor 
\[
A \otimes -: \Fil_{n} \Nil(B) \rightarrow \Fil_{n} \Nil(B)
\]
is naturally isomorphic to the functor 
\[
f \otimes -: \Fil_{n} \Nil(B) \rightarrow \Fil_{n} \Nil(B)
\]
Now we compute $\tilde{K_{0}} \Nil(C[y]/y^{n})$. Consider the following diagram:
\[
\xymatrix{
(y) \ar[rr] \ar[d] & & C[y]/(y^{n}) \ar[rr]^{y \mapsto 0} \ar[d] & & C \ar[d] \\
(y) \ar[rr] & & C[y]/(y^{n})[t] \ar[rr]^{y \mapsto 0} & &  C[t]
}
\]
Applying the functor $SK_{1}$, we get a diagram
\[
\xymatrix{
SK_{1}(C[y]/(y^{n}), (y)) \ar[rr] \ar[d] & & SK_{1}(C[y]/(y^{n})) \ar[rr]^{y \mapsto 0} \ar[d] & & SK_{1}(C) \ar[d] \\
SK_{1}  (C[y]/(y^{n})[t], (y)) \ar[rr] & & SK_{1} (C[y]/(y^{n})[t]) \ar[rr]^{y \mapsto 0} & &  SK_{1}(C[t])
}
\]
such that both rows are exact in the middle, and also on the right-hand side since the two right-hand horizontal maps split.  The two relative $SK_{1}$-groups vanish because the ideal $(y)$ is a nil ideal in both rings. The right-hand vertical map is an isomorphism because $C$ is regular. It follows that the vertical map in the middle is an isomorphism. \\
Since $\tilde{K_{0}}  \Nil(C[y]/y^{n})$ is the cokernel of the map $K_{1} (C[y]/(y^{n})) \rightarrow K_{1} (C[y]/(y^{n})[t])$, this implies that the determinant  induces an isomorphism $\tilde{K_{0}}  \Nil(C[y]/(y^{n})) \rightarrow (1+yt\Nil(C[y]/(y^{n})[t])^{\times}$.  Since a nilpotent matrix $B$ corresponds to the invertible element $1+Bt$ of $C[y]/(y^{n})[t]$, taking the determinant of $1+Bt$ corresponds (up to maybe a sign) to taking the characteristic polynomial of $B$.  So the characteristic polynomial induces an isomorphism 
\[
\tilde{K_{0}} \Nil(C[y]/y^{n}) \rightarrow  (1+yt\Nil(C[y]/(y^{n})[t])^{\times}
\]
\fxnote{details or references}


Now the characteristic polynomial of our matrix $A$ is easily computed: it is $1+x_{1}yt+x_{2}y^{2}t^{2}+x_{3}y^{3} t^{3}+...+x_{n+m}y^{n+m}t^{n+m}$. Since $y^{n} = 0$, this only depends on $x_{1}, ...x_{n-1}$, so we may replace $A$ with the matrix
\[
A = y\begin{pmatrix}
0 & 0 & 0 & ... & 0 \\
1& 0& 0&... & 0 \\
0 & 1& 0 & ...& ... \\
... & ... &... & ... & ... \\
0 & 0 & 0 &... & 0 \\
0 & 0 & 0 &... & -x_{n-1} \\
... & ... &... & ... & ... \\
0 & 0 & 0 &...&-x_{1}
\end{pmatrix} 
\]
without changing its $\tilde{K_{0}}$-class. The same argument applies to $g$, hence $f$ and $g$ induce the same map on $\tilde{K_{*}} \Fil_{n} \Nil(B)$ and their difference acts as $0$.
\end{proof}

\begin{cor}
The $\bend_{0}(R)$-action on $\tilde{K_{*}} \Nil(B)$ extends to an action of the Witt ring $W(R)$. 
\end{cor}

\begin{proof}
We have just checked continuity of the action, hence it extends to the completion.
\end{proof}

\subsection{Generalized Nil groups}

\fxnote{do it}





==> chapters/functor.tex <==
\section{A functor to spectra}















==> misc/CV.tex <==
\bigskip

\begingroup
\let\clearpage\relax
\let\cleardoublepage\relax
\let\cleardoublepage\relax
\chapter*{Lebenslauf}
For reasons of data protection, the curriculum vitae is not included
in the online version

\endgroup






==> misc/ESTA.tex <==
R199RX8RRB7F2CQF

==> misc/erkla__rung.tex <==
\fancypagestyle{plain}{}
 
Ich versichere hiermit, dass ich die vorliegende Doktorarbeit selbststŠndig, ohne unzulŠssige
 
Hilfe Dritter und ohne Benutzung anderer als der angegebenen Hilfsmittel angefertigt habe.
 
\vspace*{1.5cm}
 
Berlin, den \today
 
\vspace*{2.5cm}
 
Fabian Lenhardt






==> misc/erklaerung.tex <==
\pagebreak 



\noindent{Ich versichere hiermit, dass ich die vorliegende Doktorarbeit selbstst\"andig, ohne unzul\"assige Hilfe Dritter und ohne Benutzung anderer als der angegebenen Hilfsmittel angefertigt habe.}
 
\vspace*{1.5cm}
 
Berlin, den 
 
\vspace*{2.5cm}
 
Fabian Lenhardt





